Harnessing LLM to Attack LLM-Guarded Text-to-Image Models

To prevent Text-to-Image (T2I) models from generating unethical images, people deploy safety filters to block inappropriate drawing prompts. Previous works have employed token replacement to search adversarial prompts that attempt to bypass these filters, but they have become ineffective as nonsensical tokens fail semantic logic checks. In this paper, we approach adversarial prompts from a different perspective. We demonstrate that rephrasing a drawing intent into multiple benign descriptions of individual visual components can obtain an effective adversarial prompt. We propose a LLM-piloted multi-agent method named DACA to automatically complete intended rephrasing. Our method successfully bypasses the safety filters of DALL-E 3 and Midjourney to generate the intended images, achieving success rates of up to 76.7% and 64% in the one-time attack, and 98% and 84% in the re-use attack, respectively. We open-source our code and dataset on [this link](https://github.com/researchcode003/DACA).

==> sec/2_prelims.tex <==
\section{Preliminaries}
In this section, we illustrate two essential concepts in the attack-defense warfare of T2I models: safety filters and adversarial prompts. 

\if 0
\begin{figure*}[t]
    \centering    
    \includegraphics[width=0.9\linewidth]{figure/boundary.pdf}
    \caption{\small Two semantic boundaries enforced by LLM-assisted safety filters in T2I models: (a) illustrates the semantic safe/unsafe boundary $\mathcal{B}_s$; (b) demonstrates the existence of adversarial prompts that bypasses the safe/unsafe boundary while maintaining embedding similarity with a harmful prompt; (c) shows the semantic logical/illogical boundary $\mathcal{B}_l$, which filters out illogical prompts; (d) highlights our goal to find safe and logical adversarial prompts that can bypass two boundaries of the LLM-assisted safety filter and fall within a similar visual semantic space as a harmful prompt.}
    \label{fig-attack_modeling}
\end{figure*}
\fi 

\subsection{Safety Filter}

T2I models' safety filters mainly fall into two categories based on their position in the overall image generation chain: pre-generation filters and post-generation filters.

Pre-generation filters, also called text-based filters, operates on the rationale that the embedding space between text and images is aligned during T2I model training. Thus, it analyzes the content of input prompts to prevent the generation of inappropriate images. 
Post-generation filters, also known as image-based filters, examine the output image directly. However, compared to pre-generation filters, they incur higher costs due to the need for more image generation. Additionally, image understanding is generally more challenging than pure text understanding. Therefore, \textbf{pre-generation (text-based) safety filters, as shown in Figure~\ref{fig-t2imodel}, remain the most commonly used in practice}. Within text-based filters, existing works include two mainstream techniques: \textbf{basic safety filters} and \textbf{LLM-assisted safety filters}.

\textbf{Basic Safety Filters}. 
The representative ones are those used in open-source solutions~\cite{li2022nsfw} and DALL·E 2~\cite{dalle2}. 
These can be regarded as first-generation safety filters, relying on (i) Blocklists: They curate a list of harmful words, and when an input prompt matches an entry on this list, the associated image generation request is denied. 
% The word lists could be public~\cite{} or maintained by specific organizations.
(ii) Prompt Classifiers: 
They primarily utilize frozen models like CLIP~\cite{clip_repo} to classify the content of text into predefined categories. These categories typically include hate, threats, self-harm, sexual content, minors, and violence. For example, an open-source binary classifier~\cite{li2022nsfw} adopts the DistilBERT~\cite{sanh2019distilbert} model, fine-tuned on data collected from an NSFW content channel on Reddit. The moderation Policy~\cite{dalle2_moderation} used by DALL·E 2 adopts a similar principle.
% Such classifiers are available in both open-source and proprietary versions. 

\textbf{LLM-assisted Safety Filters}. The representative examples are those used in DALL·E 3~\cite{dalle3} and MidJourney V6~\cite{midjourney}. These systems incorporate LLMs, such as ChatGPT~\cite{gpt4,chatgpt}, to conduct text filtering. Due to the enhanced text understanding capabilities of LLMs, LLM-assisted filters can effectively block harmful text based on system-prescribed instructions.
In practice, the LLM will either refuse to execute the drawing intent or clean the prompt by removing inappropriate words. Additionally, LLMs will reject chaotic or illogical inputs, which are often challenging for basic safety filters to handle accurately.


% In current text-to-image conversion technology, mainstream methods typically use text-based detection mechanisms for reasons of cost and efficiency. This mechanism works by analyzing the input text prompts to intercept the generation of images containing harmful content. Specifically, during the training phase, the model converts text prompts and corresponding image concepts into vector form and maps them within a high-dimensional embedding space. This vector mapping allows safety filters to prevent the generation of inappropriate images based solely on whether the text contains harmful information.

% While image content-based detection methods also exist, they are often not prioritized due to their higher cost and less stable detection results. Based on our testing and practical experience, these image-based detection systems have not achieved the high efficiency and accuracy claimed by some manufacturers. Therefore, in practical applications, text filters remain the most commonly used and effective means to prevent the generation of images containing harmful content. 

% Currently, text filters employ two mainstream technological approaches for text detection. The first is represented by open-source detectors and DALL·E 2, which are first-generation "black box" detectors primarily based on preset rules and keywords, with limited user understanding of their internal logic.

% The second-generation detectors, such as those released with DALL·E 3 and MidJourney V6, incorporate Large Language Models (LLMs) like ChatGPT to assist in text detection. This new generation of detectors, known as LLM-assisted safety filters, make significant improvements over the architecture of basic detectors by combining traditional text filtering techniques with advanced language understanding capabilities, enhancing recognition of complex and subtle semantics. The LLM-assisted method can identify not only obvious violations but also understand potentially inappropriate content within the context, thus providing more in-depth and accurate safety filtering.

% In this paper, we define detectors based on early simple rules as "basic safety filters" and those enhanced with LLM as "LLM-assisted safety filters."

% \subsubsection{Basic Safety Filter}
% Basic detectors can primarily be divided into two types:

% \textbf{Prompt Input Classifiers.} These detectors mainly utilize frozen models like CLIP to classify text content by calculating the similarity between input text and predefined categories. These categories include, but are not limited to, hate, threatening, self-harm, sexual content, minors, and violence. Such classifiers are available in both open-source and proprietary versions. For example, an open-source version could involve a binary classifier fine-tuned on data collected from a NSFW content channel on Reddit using DistilBERT. Proprietary versions include the Moderation API used by the DALL·E series TTI engines provided by OpenAI.

% \textbf{Blocklists.} This detection mechanism is more direct and relies on a pre-collected and defined list of harmful prompts. When a user's input text matches an entry on this list, the related image generation request is automatically denied. These lists are often public, such as the “nsfw\_list” on GitHub, but can also be private, maintained by specific organizations or projects.

% \subsubsection{LLM-assisted Safety Filter}
% With the rapid development of LLMs, these models are increasingly being applied in TTI conversion technologies to enhance security measures. LLMs demonstrate their deep understanding capabilities when processing user input prompts, conducting detailed analysis of the text, and effectively blocking and filtering harmful content based on system-prescribed rules.

% In practice, an LLM first parses and understands the input prompt, and then identifies harmful or inappropriate content based on the standards set by the system. Upon detecting such content, the LLM employs strategies to disassemble and rewrite the prompt, replacing sensitive or inappropriate words while transforming the prompt into a clearer format that meets the requirements of the drawing engine. The processed content is not only safer but also more comprehensible and executable in the subsequent image generation process.

% After the initial processing by the LLM, the modified prompt is still sent to the basic safety filter for further inspection to ensure all potential risks are thoroughly eliminated. Additionally, due to the LLM's strong semantic understanding capabilities, it can effectively recognize and reject chaotic or meaningless inputs, which are often challenging for traditional methods to accurately handle. For example, for prompts that are structurally chaotic and lack practical meaning, the LLM can directly deem them as invalid inputs and reject them.



% \begin{figure*}[t]
%     % \centering
%     % \includegraphics[width=0.98\linewidth]{figure/bypass_rate_dalle_onetime.jpg}
%     % \caption{\textcolor{red}{todo}}
%     % \label{fig:eval_bypass_dalle}
%     \centering
%     \begin{subfigure}{0.24\linewidth}
%         \includegraphics[width=\linewidth]{figure/modeling_a.png}
%         \caption{}
%         \label{fig:(a)}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}{0.24\linewidth}
%         \includegraphics[width=\linewidth]{figure/modeling_b.png}
%         \caption{}
%         \label{fig:(b)}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}{0.24\linewidth}
%         \includegraphics[width=\linewidth]{figure/modeling_c.png}
%         \caption{}
%         \label{fig:(c)}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}{0.24\linewidth}
%         \includegraphics[width=\linewidth]{figure/modeling_d.png}
%         \caption{}
%         \label{fig:(d)}
%     \end{subfigure}
%     \caption{Model of the relationship between semantic security boundaries and semantic accuracy boundaries with the embedding space of prompts.}
%     \label{fig:attack_modeling}
% \end{figure*}



\subsection{Adversarial Prompts}
Adversarial inputs, where attackers strategically manipulate the input to trigger unintended outputs in AI models, have attracted significant attention in recent years. The initial focus was on the computer vision domain~\cite{goodfellow2014explaining, carlini2017towards, kurakin2018adversarial}, where subtle perturbations, imperceptible to human eyes, were introduced to images to mislead model classification. 
% into making incorrect decisions, such as erroneous classification.
This concept has been observed in other continuous modalities like time-series signals~\cite{han2020deep, chen2020ecgadv} and discrete ones like natural language texts~\cite{li2018textbugger, jin2020bert, garg2020bae}. 

In text domain, earlier studies~\cite{li2018textbugger, garg2020bae} primarily aimed to deceive text classification models. 
% \eg, replacing certain words/tokens using synonyms to maintain original semantics while altering the model's decision. 
% TextBugger~\cite{li2018textbugger} demonstrated that manipulating key words through swapping, removing, or substituting can significantly alter predictions while minimally impacting human comprehension. 
% Jin \etal.\cite{} proposed rule-based synonym replacement strategies for crafting more natural-looking adversarial examples, aiming to maintain semantic similarity to the original text while passing human scrutiny. 
% BAE~\cite{garg2020bae} suggests masking parts of the text and employing a BERT masked language model to generate semantically coherent adversarial text replacements.
% Earlier studies primarily aimed to deceive text classification models. 
% into incorrect results, like causing a spam detector to fail at identifying spam emails. 
However, with the rising popularity of T2I models, recent research has begun to explore adversarial prompts to generate unintended images. Milliere \etal.\cite{milliere2022adversarial} showed that attackers could create adversarial examples by combining words from different languages against T2I models. Maus \etal.\cite{maus2023adversarial} developed a black-box framework using Bayesian optimization for adversarial prompt generation, aiming to generate images of a target class using nonsensical tokens. 
Rando \etal.\cite{rando2022red} and Qu \etal.\cite{qu2023unsafe} proposed adversarial strategies like prompt dilution to break safety filter of Stable Diffusion~\cite{rombach2022high}. A recent work~\cite{yang2023sneakyprompt} employed reinforcement learning method to search and replace sensitive tokens by repeatedly querying T2I models, which circumvented closed-box safety filters in \dalle~2~\cite{dalle2} to generate sexual images. 
These works are successful to bypass basic safety filters, but they fail to bypass LLM-assisted ones adopted in the latest T2I models.


==> sec/3_boundary-model.tex <==
% \section{Detection Methodology}
\section{Filtering Boundary Formalization}
\label{sec-boundary}



In this section, we will formally illustrate two important filtering boundaries employed by existing text-based safety filters: the semantic safe/unsafe boundary and the semantic logical/illogical boundary. We then describe threat model used in this work. 

\textbf{Semantic Safe/Unsafe Boundary}.
The safety filters of T2I models, whether basic or LLM-assisted ones, will implicitly perform a binary classification of the drawing prompt as either safe/harmless or unsafe/harmful as shown in Figure~\ref{fig-attack_modeling}(a). Technically, they transform text $T$ into vectors $\mathbf{v}$ and set a semantic safe/unsafe boundary $\mathcal{B}_s$ in the embedding space. This boundary determines which text vectors are safe and which may lead to the generation of harmful images, which can be described by $\mathcal{B}_s:f_s(\mathbf{v})=0$, where $f_s(\mathbf{v})$ demonstrates the safety score of the vector $\mathbf{v}$ in relation to the semantic safety boundary $\mathcal{B}_s$. Therefore, the positive space, which represents the safe space, can be expressed as  $\mathcal{P}_s=\{\mathbf{v} \in \mathbb{R}^{n \times 1}|f_s(\mathbf{v})>0\}$. Conversely, the negative space, representing the potentially unsafe space, can be defined as $\mathcal{N}_s=\{\mathbf{v} \in \mathbb{R}^{n \times 1}|f_s(\mathbf{v})<0\}$.

However, this boundary has been empirically proven to be imperfect. 
Some harmful text embeddings could fall on the safe side $\mathcal{P}_s$, leading to erroneous classification, as shown in Figure~\ref{fig-attack_modeling}(b). Prior work~\cite{yang2023sneakyprompt} has shown that such adversarial prompts could be efficiently searched. Specifically, they utilize reinforcement learning framework to replace sensitive tokens in the original prompts to find text with vector $\mathbf{v}_{a} = \{\mathbf{v}|\mathbf{v} \in \mathcal{P}_s\}$. 
% For example, the prompt word "naked" can be altered to "mambo incomplete clicking". 
For example, the prompt word "penis" can be replaced by "iminjymaisw". 
Their embedding are close, but the latter falls on the safe side $\mathcal{P}_s$, making  DALL·E 2 generating inappropriate images. 

\textbf{Semantic Logical/Illogical Boundary}. Besides the semantic safe/unsafe boundary, LLM-assisted safety filters, adopted by most advanced T2I models like DALL·E 3 and MidJourney, demand higher standards for prompts: only drawing prompts that can be understood may proceed to image generation. This implicitly introduces an additional boundary, the semantic logical/illogical boundary $\mathcal{B}_l$, as shown in Figure~\ref{fig-attack_modeling}(c).  
Similarly, the positive space, which represents the comprehensible space, can be expressed as $\mathcal{P}_l=\{\mathbf{v} \in \mathbb{R}^{n \times 1}|f_l(\mathbf{v})>0\}$, and the negative space, representing the incomprehensible space, can be defined as $\mathcal{N}_l=\{\mathbf{v} \in \mathbb{R}^{n \times 1}|f_l(\mathbf{v})<0\}$. $f_l(\mathbf{v})$ represents the logical score of the vector $\mathbf{v}$ in relation to the semantic logical/illogical boundary $\mathcal{B}_l$. For example, the prompt "iminjymaisw" mentioned earlier falls on the safe side $\mathcal{P}_s$ of semantic safe/unsafe boundary, which pass through the basic safety filters, but because its expressed semantics are not logical enough to be understood by the LLM, it fails to pass the semantic logical/illogical boundary $\mathcal{B}_l$, and thus cannot pass through the LLM-assisted safety filter.
In another word, a vector $\mathbf{v}$ that meets the condition $\mathbf{v} \in \mathcal{P}_s$ can pass the basic safety filter, while it needs to meet the condition $\mathbf{v} \in \mathcal{P}_s \cap \mathcal{P}_l$ to pass the LLM-assisted safety filters.

% \subsection{Detection Boundary}
% \textbf{Semantic Safety Boundary}
% Continuing with the analysis of basic safety filters from the SneakyPrompt paper, in the design of safety filters for text-to-image engines, the foundational safety filters - including prompt input classifiers and blocklists - essentially perform a binary classification of text into "harmful" or "harmless". This classification is achieved by transforming text $T$ into vectors $\mathbf{v}$ and setting a semantic safety boundary $\mathcal{B}_s$ in the embedding space. This boundary determines which text vectors are safe and which may lead to the generation of harmful images, which can be described by $\mathcal{B}_s:f_s(\mathbf{v})=0$, where $f_s(\mathbf{v})$ demonstrates the safety score of the vector $\mathbf{v}$ in relation to the semantic safety boundary $\mathcal{B}_s$. Therefore, the positive space, which represents the safe space, can be expressed as  $\mathcal{P}_s=\{\mathbf{v} \in \mathbb{R}^{n \times 1}|f_s(\mathbf{v})>0\}$. Conversely, the negative space, representing the potentially harmful space, can be defined as $\mathcal{N}_s=\{\mathbf{v} \in \mathbb{R}^{n \times 1}|f_s(\mathbf{v})<0\}$.

 
% The establishment of a semantic safety boundary $\mathcal{B}_s$ in the embedding space can be likened to a planar structure, intersecting with a spherical region $\mathcal{C}$ representing harmful concepts. For example, consider a harmful concept $c_p$ representing pornographic content, abstracted in the embedding space as a spherical region $\mathcal{C}_p$ where all included string vectors $\mathbf{v}_{c_p}$ possess potential pornographic meanings $c_p$. If this sphere intersects with the semantic safety boundary $\mathcal{B}_s$, some string vectors capable of expressing concept will fall on the safe side $\mathcal{P}_s$, leading to their erroneous classification as "safe". 
\if 0
This security vulnerability is particularly susceptible in adversarial prompt attacks, where algorithms like SneakyPrompt, representing adversarial prompt search, can easily find prompts that circumvent the semantic safety boundary $\mathcal{B}_s$. They employ reinforcement learning, rewarding the similarity between adversarial and original prompts and their ability to pass the basic safety filters, by altering some characters in the original prompts to find strings that can bypass the basic safety filters - these strings are the discovered adversarial prompts $\mathbf{v}_{ad} = \{\mathbf{v}|\mathbf{v} \in \mathcal{P}_s\}$.
\fi 

% For instance, when a prompt word such as “naked” is positioned on the harmful side $\mathcal{N}_s$ due to its direct implication of potential pornographic content, the security filter would block this prompt. However, a semantically similar but differently phrased prompt "mambo incomplete clicking", due to subtle semantic differences, would be placed on the safe side $\mathcal{P}_s$ of the safety boundary $\mathcal{B}_s$, thereby bypassing the security filter and ultimately allowing the generation of images with similarly harmful meanings.


% \textbf{Semantic Precision Boundary}
% As artificial intelligence continues to advance in the field of security, the application of LLMs is gradually expanding into more complex domains of security detection. OpenAI, with the launch of its latest generation text-to-image engine, DALL·E 3, was the first to integrate LLMs into its safety defense mechanisms. This approach was soon adopted by other TTI engine service providers, such as Midjourney, who introduced LLM-assisted safety detection mechanisms to enhance product security performance.

% The LLM-assisted safety filter is a second-generation security filter developed from basic safety filters. This new type of safety filter relies on the LLM's deep understanding capabilities of prompts inputted into TTI engines. The text filtering process involves two main stages: text understanding and text transformation.

% During the text understanding stage, the LLM transforms the input prompt $T$ into embedding vectors $\mathbf{v}$ and interprets its meaning based on preset system parameters. At this stage, the LLM actively checks whether the input contains harmful content. If the system determines that the input contains harmful content or is difficult for the LLM to understand, the engine service request for this input will be blocked, effectively intercepting harmful content. Following text understanding, the text transformation stage begins, where the LLM performs more detailed content expansion and standardizes the formatting to optimize the input for the drawing engine.

% % Building on the basic "semantic safety boundary $\mathcal{B}_s$" for textual harmfulness, the LLM-assisted safety filter, in its first "text understanding" stage, demands higher standards for prompts: only language that can be understood may pass. This is abstracted as a "semantic precision detection boundary $\mathcal{B}_p$" similar to the "semantic safety boundary $\mathcal{B}_s$", maintained through functions to ensure the semantic accuracy and appropriateness of the input prompts. Similarly, the positive space, which represents the comprehensible space, can be expressed as $\mathcal{P}_p=\{\mathbf{v} \in \mathbb{R}^{n \times 1}|f_p(\mathbf{v})>0\}$, and the negative space, representing the incomprehensible space, can be defined as $\mathcal{N}_p=\{\mathbf{v} \in \mathbb{R}^{n \times 1}|f_p(\mathbf{v})<0\}$. $f_p(\mathbf{v})$ represents the precision score of the vector $\mathbf{v}$ in relation to the semantic precision boundary $\mathcal{B}_p$. For example, as mentioned earlier with SneakyPrompt, the prompt "naked", due to its potential pornographic meaning, would be deemed to fall on the harmful side $\mathcal{N}_s$ of the safety boundary and thus be blocked. "Mambo incomplete clicking" falls on the safe side $\mathcal{P}_s$ of the semantic safety boundary that can pass through the basic safety filter, but because its expressed semantics are not precise enough to be understood by the LLM, it fails to pass the semantic precision boundary $\mathcal{B}_p$, and thus cannot pass through the LLM-assisted Safety Filter.

% Abstractly speaking, a vector $\mathbf{v}$ that meets the condition $\mathbf{v} \in \mathcal{P}_s$ can pass the basic safety filter, while it needs to meet the condition $\mathbf{v} \in \mathcal{P}_s \cap \mathcal{P}_p$ to pass the LLM-assisted safety filter.

\if 0
Furthermore, the reward functions of adversarial prompt search algorithms only consider vector-level similarity, resulting in adversarial prompts and their derivatives being merely in compliance with basic safety filter restrictions, rather than natural language prompts intended for human understanding. These prompts, often due to the lack of recognizable and interpretable meaning by LLMs, are blocked. Notably, these character-stacked prompts may in rare cases indeed be real words, but the meaning of these words is far removed from the original harmful content, so even if they occasionally pass through the semantic precision boundary $\mathcal{B}_p$, they lose their initially harmful semantic intent.
\fi 

\textbf{Threat Models}. 
The attack goal here is to induce a T2I model equipped with an LLM-assisted safety filter to generate inappropriate images. Technically, for a given drawing prompt $T$ that would originally be blocked, we intend to find an adversarial version $T_a$ with an associated embedding vector $\mathbf{v}_a$ as shown in Figure~\ref{fig-attack_modeling}(d). 
This attack procedure has two steps: bypass and expose. The bypass step focuses on whether the prompt can pass through the safety filter without being intercepted, \ie, $\mathbf{v}_a \in \mathcal{P}_s \cap \mathcal{P}_l$. 
The expose step requires $\mathbf{v}_a$ to fall within a similar visual semantic space as the original prompt $T$, \ie, the T2I model can generate images containing the intended content.
% concerns whether the T2I model can generate images containing harmful content.
Prompts that merely pass through the safety filter but fail to display harmful content in the image are regarded as failures, while only when both bypass and expose are achieved can it be considered a successful jailbreak of LLM-assisted safety filter.

% that satisfies  $\mathbf{v}_a \in \mathcal{P}_s \cap \mathcal{P}_l$, as shown in Figure~\ref{fig-attack_modeling}(d). 
% This jailbreaking procedure can be regarded as two steps: bypass and expose. The bypass step focuses on whether the prompt can pass through the safety filter without being intercepted, while the expose step concerns whether the T2I model can generate images containing harmful content.


% \textcolor{red}{todo: do we assume not interact with online T2I model?} No


% Our goal is to induce a text-to-image generation engine to produce images that its safety rules explicitly prohibit. We define this operation as "Jailbreak LLM-assisted Safety Filter". We propose a comprehensive jailbreaking framework that includes two key steps: bypass and expose. The bypass step focuses on whether the input prompt can pass through the safety filter without being intercepted; the expose step concerns whether the TTI engine can generate images containing harmful content after receiving the input prompt. Previous research often considered the successful passage of adversarial prompts through safety filters as a successful jailbreak, which corresponds to our defined first step, bypass, but neglected whether these prompts truly achieve the goal of expressing harmful semantics in the output images. We believe that prompts that merely pass through the safety filter but fail to display harmful content in the image are actually a failure. Therefore, our framework considers that only when both bypass and expose are achieved can it be considered a successful jailbreak of the LLM-assisted safety filter.

\if 0
\subsection{Adversarial Attack Modeling}
Based on the analysis of semantic safety boundaries and semantic accuracy boundaries, we model the Adversarial Attack targeting the LLM-assisted Safety Filter. The LLM-assisted Safety Filter filters input prompts using two boundaries: a semantic safety boundary and a semantic accuracy boundary. In the embedding space, we conceptualize the semantic safety boundary as a plane M1, depicted as the blue colored plane in figure~\ref{fig:attack_overview}. This plane divides the entire embedding space into harmful and harmless sections. Similarly, we abstract the semantic accuracy boundary of the safety filter as another plane, M2, shown as yellow plane in the figure~\ref{fig:attack_overview}, which bifurcates the embedding space into accurate and inaccurate sections. We consider the distribution of vectors representing any harmful semantic in the embedding space as a sphere; all prompts within this sphere can express that harmful semantic, as illustrated by the grey sphere in figure~\ref{fig:attack_overview}. A prompt can pass through the LLM-assisted Safety Filter if its corresponding vector in the embedding space is simultaneously on the harmless side of M1 and the accurate side of M2. The intersection of these two planes forms the safe space allowed by the LLM-assisted Safety Filter for passing prompts. Therefore, to generate adversarial prompts containing harmful semantics, the spherical space formed by vectors expressing these semantics must intersect with the safe space.

This explains why previous search algorithms failed to produce adversarial prompts that could bypass the LLM-assisted Safety Filter: The reward functions of adversarial prompt search algorithms only consider vector-level similarity, resulting in prompts that meet only the basic safety filter's restrictions—these are feature-conforming rather than naturally understandable language prompts. Often, these prompts are blocked because they lack meanings that LLMs can recognize and interpret. Notably, these stacked character prompts might, in rare cases, constitute actual words in reality, but their meanings are far removed from the original harmful content. Thus, even if they occasionally pass the semantic accuracy boundary, they lose their initially harmful semantic intent.
\fi 

==> sec/4_enhancerl.tex <==
\section{Search-and-Replace Adversarial Prompt Generation}
\label{sec-sneakp}

% \begin{figure*}[t]
%     \centering \includegraphics[width=\linewidth]{figure/Improve_SneakyP.png}
%     \caption{\small The algorithm improved on the sneakyprompt.}
%     \label{fig-improve_sneakyp}
% \end{figure*}

% \label{compare}
% \begin{figure}[t]
%     \centering \includegraphics[width=\linewidth]{figure/Compare.png}
%     \caption{\small The relationship between adversarial examples searched by SneakyPrompt and DACA.}
%     \label{fig-compare}
% \end{figure}

\begin{figure}[t]
    \centering \includegraphics[width=\linewidth]{figure/search-and-place.pdf}
    \caption{\small Search-and-Replace Adversarial Prompt Generation. We implement and evaluate two types of amendments: 1) incorporating a safety filter with a logical/illogical boundary into system environment; 2) incorporating a semantic logic score into reward function.}
    \label{fig-improve_sneakyp}
\end{figure}

This section describes our attempt to explore potential ways to amend and enhance the prior search-and-replace strategy to bypass the LLM-assisted safety filter of DALL·E 3.

\textbf{Basic Principle of Search-and-Replace Method}. Figure~\ref{fig-improve_sneakyp} provides a simplified overview of the search-and-replace method used to generate adversarial prompts. The process involves two main components: Sampler and System Environment. The Sampler executes the search-and-replace strategy, identifying sensitive tokens in the input prompt and replacing them with insensitive ones. The System Environment typically features a T2I model with a safety filter, which accepts the generated prompts and provides feedback including block or bypass, the quality of generated images, \etc, to guide the Sampler in refining the prompts in subsequent steps.

\textbf{Amendment Attempts}. The prior search-and-replace method~\cite{yang2023sneakyprompt} used DALL·E 2 as the system environment, allowing it to bypass prompts even if they contained meaningless tokens like "iminjymaisw". Additionally, their reward function primarily focused on embedding similarity, as shown in the gray cycle in Figure~\ref{fig-attack_modeling}, without giving much consideration to whether the prompts made logical sense. Therefore, we implement two types of amendments to the vanilla method:

$\bullet$~\underline{+Semantic Logic Checking in Safety Filter}. We enhance the safety filter within the system environment to include semantic logic checking. We test two options: (a) utilizing an English dictionary~\cite{nltk} and developing a simple checking logic to ensure that each word in the generated prompt is valid. (b) leveraging the LLM (GPT-4)-assisted filter, as used by DALL·E 3, as a semantic logic checker.

$\bullet$~\underline{+Semantic Logic Scoring in Reward Function}. We enhance the reward function by incorporating semantic logic scoring. We test two approaches: (a) calculating the perplexity~\cite{jelinek1977perplexity} of the prompt to assess its logical coherence. Perplexity is a standard metric for evaluating language fidelity. By computing the average perplexity of all words from the NLTK dataset~\cite{nltk}, along with their altered forms (generated by adding, deleting, or flipping characters), we observe that real vocabulary tends to have lower perplexity, while artificially altered and confusing vocabulary shows higher perplexity. Thus, perplexity can partially indicate whether text content is logical and meaningful. (b) utilizing the GPT-4 API~\cite{gpt4} to score the logical coherence and clarity of generated prompts. These scores are scaled and integrated into the original embedding similarity-based reward function.


% method has three key components: Prompt Sampler, Safety Filter (Proxy), and Reward Function. Prompt Sampler is responsible for altering the original prompt to generate candidates for adversarial prompts. Safety Filter (Proxy) serves as an environment to check whether the candidate can successfully bypass the filter. Reward Function guides Prompt Sampler to find better candidates. 

% In this section, we analyze the state-of-the-art RL-based adversarial prompt search method, SneakyPrompt, and examine the reasons for its failure against LLM-assisted safety filters. We then explore the possibility of improving it to successfully bypass the LLM-assisted safety filter of DALL·E 3.

% \textbf{Basic Principle of RL-based Method}. As shown in Figure~\ref{fig-improve_sneakyp}, the RL-based method has three key components: Prompt Sampler, Safety Filter (Proxy), and Reward Function. Prompt Sampler is responsible for altering the original prompt to generate candidates for adversarial prompts. Safety Filter (Proxy) serves as an environment to check whether the candidate can successfully bypass the filter. Reward Function guides Prompt Sampler to find better candidates. 

% This explains why previous search algorithms failed to produce adversarial prompts that could bypass the LLM-assisted Safety Filter: The reward functions of adversarial prompt search algorithms only consider vector-level similarity, resulting in prompts that meet only the basic safety filter's restrictions—these are feature-conforming rather than naturally understandable language prompts. Often, these prompts are blocked because they lack meanings that LLMs can recognize and interpret. Notably, these stacked character prompts might, in rare cases, constitute actual words in reality, but their meanings are far removed from the original harmful content. Thus, even if they occasionally pass the semantic accuracy boundary, they lose their initially harmful semantic intent.

% \textbf{Prior Work Analysis}. In previous RL-based methods~\cite{}, Reward Function only considers embedding-level similarity with the original prompt. They do not guarantee that the resulting prompt preserves logical meaning. As a result, the LLM may treat these prompts as nonsensical sentences and refuse to generate an image. These stacked character prompts might have real words, but their surface meanings are far away from the original intent. Thus, even if they occasionally pass the semantic accuracy boundary, they lose their initial intent.

% \textbf{Incorporating Semantic Logic}. Here, we explore the possibility of integrating the two semantic boundaries stated in \S\ref{sec-boundary} into the RL-based methods mentioned above, so that we can find effective adversarial prompts that meet the condition $\mathbf{v} \in \mathcal{P}_s \cap \mathcal{P}_l$ to pass the LLM-assisted safety filter. Specifically, we introduce semantic logic/illogical checker to enhance both Safety Filter (Proxy) and Reward Function. We adopt two types of checkers, as shown in Figure~\ref{fig-improve_sneakyp}.

% \noindent\underline{LLM as Logic Checker}. Here, we utilize the GPT-4 API to check and score the inherent logical coherence and understandability of the input. This score is then scaled and added to the Reward Function.

% \noindent\underline{Perplexity as Logic Checker}. Here, we adopt Perplexity~\cite{} as a metric to quantify the logical coherence of the input. Perplexity is commonly used to measure language fidelity. By calculating the average perplexity of all words from the NLTK words dataset~\cite{}, along with their morphed forms obtained through adding, deleting, or flipping characters, we found that actual vocabulary typically has lower perplexity, while artificially altered, confusing vocabulary shows higher perplexity. Therefore, using perplexity can, to some extent, assess whether the text content is logical and meaningful. We also incorporate this metric into Reward Function.

The above amendments aim to encourage the generation of effective adversarial prompts that still preserve logical meaning.



\begin{table}[t]
\caption{Results of Amended Search-and-Replace Prompt Generation.}
\centering
\resizebox{\linewidth}{!}{%
\begin{tabular}{|c|c|c|}
\hline
& Search-and-Replace+X & Success? \\ \hline
\multirow{2}{*}{+semantic logic filter} & dictionary-based filter & \usym{2718}      \\ \cline{2-3}
& LLM-based filter & \usym{2718}      \\ \hline
\multirow{2}{*}{+semantic logic score} & perplexity-based score & \usym{2718}       \\ \cline{2-3}
& LLM-based score & \usym{2718}       \\ \hline
\end{tabular}%
}
\label{tab-settings_search_results}
\end{table}

\textbf{Empirical Evaluation and Results}. We use our curated harmful prompt dataset, as detailed in \S~\ref{sec-eval-setting}, for evaluation. The results are presented in Table~\ref{tab-settings_search_results}. 
In terms of upgrading the safety filter to include semantic logic checks in the system environment, whether using dictionary-based or LLM-based filter, we found that after more than 1,000 search iterations, no valid adversarial prompts were generated. This is because the search-and-replace strategy, illustrated in Figure~\ref{fig-improve_sneakyp}, fails to produce prompts where all words are valid. Consequently, the system environment consistently returns a "block" response, providing the Sampler with insufficient feedback for improvement. When semantic logic scoring is applied, it also did not result in the generation of effective prompts capable of bypassing LLM-assisted safety filter.

Based on our analysis and experiments, we found that the search-and-replace method inherently struggles to ensure the logical coherence of the generated prompts, even with extra amendment. This is because the process, which relies on embedding similarity to select a few non-sensitive tokens to replace a sensitive one, often constructs prompts that lack logical sense. Therefore, we seek to go beyond the conventional search-and-replace prompt generation to explore LLM-based adversarial prompt generation.

% Two possibilities arise from these results: The first is that only a few original harmful prompts have their spherical space of expressed harmful semantics intersect with the safe space, indicating that only a few original harmful prompts have the potential for "harmless and accurate" strings in space. The second possibility is that the search space of these algorithms, merely flipping the original prompt's harmful words, is too small in terms of word length, resulting in incomplete adversarial prompts.

% \noindent\underline{Settings}. 
% \noindent\underline{Result Analysis}. 


% \begin{table}[h]
% \caption{Experiment results of improved sneakyprompt.}
% \centering
% \resizebox{\linewidth}{!}{%
% \begin{tabular}{|c|c|c|}
% \hline
% \multicolumn{2}{|c|}{Settings} & Search Results \\ \hline
% \multirow{5}{*}{Sneaky Prompt with} & None                             & Success        \\ \cline{2-3}
%                                     & nltk Dictionary as Discriminator & not found      \\ \cline{2-3}
%                                     & GPT-4 as Discriminator           & not found      \\ \cline{2-3}
%                                     & GPT-4 as Reward Fun              & not pass       \\ \cline{2-3}
%                                     & Perplexity as Reward Fun         & not pass       \\ \hline
% \end{tabular}%
% }
% \label{tab:settings_search_results}
% \end{table}



% The algorithm represented by SneakyPrompt involves reversing the characters in nsfw words to search for adversarial prompts, so we can consider its search space to be the size of nsfw words. Taking the nltk dataset as an example, the average English word therein contains 9.55 characters. After increasing or decreasing the number of characters on average, we can consider the original search space of SneakyPrompt to average 9.55 characters. The DACA algorithm involves replacing nsfw words and providing more detailed descriptions, and if we wish to search for adversarial prompts similar to those from the DACA algorithm using the improved SneakyPrompt algorithm, we need to utilize the improved SneakyPrompt algorithm within the search space of the DACA algorithm. We can consider the prompt obtained by the DACA algorithm as its search space, which averages 1167 characters (using the DACA algorithm on the vbcde-100 dataset with GPT-3.5/4 and other LLMs as the backbone models). 

% For the SneakyPrompt algorithm, the reversal space for each character is the 26 letters of the alphabet minus the original letter which is 25, hence the complexity of the SneakyPrompt algorithm performing a search in its basic search space is $25^{9.55}$, and the complexity of the SneakyPrompt algorithm performing a search in the DACA algorithm's search space is $25^{1167}$. Therefore, the difficulty of the improved SneakyPrompt algorithm in searching for adversarial prompts similar to those of the DACA algorithm is $25^{1167/9.55} = 25^{122.2}$ times that of the original SneakyPrompt algorithm.

% To further analyze the difficulty of the improved SneakyPrompt algorithm in searching within the DACA algorithm's search space, we conducted a reinforcement learning search on a server with an A6000 GPU using the stableDiffusion model, with a security filter being the text-image filter built into stableDiffusion. The average time to search for an nsfw word in the nsfw\_list dataset once is 6 seconds. According to the evaluation table in the SneakyPrompt article, it takes an average of 9 searches to obtain an effective adversarial prompt in this setting. Thus, using the SneakyPrompt algorithm in its original search space to search for an adversarial prompt for an nsfw word takes an average of 9x6=54 seconds. Therefore, the average time spent by the improved SneakyPrompt algorithm searching in the DACA algorithm's search space to successfully find an adversarial prompt is $54x25^{122.2}$ seconds, which is an unrealistic number. This means that the reinforcement learning search algorithm represented by SneakyPrompt is unsuccessful for searching long and complex adversarial prompts.

% \textbf{Empirical Evaluation and Results}. \textcolor{red}{TODO: organize this part better, add more evaluation details. @yimo} 



% Experimental results indicated that, whether directly utilizing the large language model itself or incorporating perplexity as part of the reward to aid in the search for adversarial prompts, we failed to find effective adversarial prompts in 1,000 search attempts.

% Two possibilities arise from these results: The first is that only a few original harmful prompts have their spherical space of expressed harmful semantics intersect with the safe space, indicating that only a few original harmful prompts have the potential for "harmless and accurate" strings in space. The second possibility is that the search space of these algorithms, merely flipping the original prompt's harmful words, is too small in terms of word length, resulting in incomplete adversarial prompts.

% To address this, we selected 1,408 NSFW words from the open-source nsfw\_list dataset as our search targets, significantly increasing the likelihood that original harmful semantics fall into region X of Figure X, eliminating experimental error due to insufficient data volume. However, even with an expanded range of vocabulary, we still failed to find suitable adversarial prompts within a limited number of search attempts. Consequently, we believe that this word-flipping search method fails to break the latest LLM-assisted Safety Filter, primarily because the prompts it discovers are mostly the words of the original harmful prompts. We speculate that the short length of adversarial prompts prevents successful searches, a limitation inherent to the algorithm, while other algorithms capable of searching for longer and more complex adversarial prompts can indeed find harmful prompts.

% After analyzing why the LLM-assisted Safety Filter successfully intercepted adversarial prompts such as "SneakyPrompt," we explored whether it might be possible to improve the search strategy for adversarial prompts, starting with SneakyPrompt, to enable them to bypass this new type of safety filter and launch an attack on the TTI Engine. The key to this attack lies in simultaneously evading both the semantic safety boundary and the newly introduced semantic accuracy boundary. The original search algorithm considered the semantic safety boundary; therefore, we attempted to integrate constraints related to the semantic accuracy boundary into the search algorithm. This integration allows the algorithm to generate adversarial prompts with accurate semantics and coherent grammatical logic, enabling successful attacks.

% Previous methods satisfied the search for safety but lacked constraints for accuracy, necessitating the addition of criteria for accuracy in the auxiliary search.

% How do we integrate constraints related to the semantic accuracy boundary into the algorithm? We need to model the accuracy boundary, which we believe fundamentally involves checking whether the text input into the LLM conforms to the LLM's assessment of logic. We implemented this check in two approximate ways show on the figure~\ref{fig:attack_overview}.

% \textbf{LLM as Boundary.} Using the GPT-4 API to score the logic and comprehensibility of input prompts. This method employs GPT-4 to score the inherent logical coherence and understandability of the text. This scoring outcome is then applied as part of the reward function in the search algorithm. Under this setup, the algorithm is encouraged to find texts that are logically strong and easy to understand, thus avoiding generating logically incoherent or difficult-to-understand adversarial prompts.

% \textbf{Perplexity as Boundary.} Introducing Perplexity as a metric to assess the quality of LLM outputs, incorporating it into the reward function of the search algorithm. Perplexity is a commonly used statistical measure for evaluating the performance of language models, gauging the model’s level of surprise (i.e., uncertainty) about a series of outputs. By calculating the average perplexity of all words from the NLTK words dataset, along with their morphed forms obtained through adding, deleting, or flipping characters, we found that actual vocabulary typically has lower perplexity, while artificially altered confusing vocabulary shows higher perplexity. Therefore, using perplexity can, to some extent, assess whether the text content is logical and meaningful.

\if 0
Given that we have identified prompts that are both harmful yet accurate and harmless yet inaccurate, with the definitions of "harmful/harmless" based on the semantic safety boundary and "accurate/inaccurate" based on the semantic precision boundary, and knowing these boundaries cannot coincide, we hypothesized the existence of prompts that meet the criteria of being "harmless and accurate." According to our previous analysis, such prompts can successfully bypass both types of safety filters and execute an attack on the TTI Engine.

In pursuit of such "harmless and accurate" prompts, we explored the semantic accuracy boundary of the algorithm using the two different implementation methods previously described, and made improvements to SneakyPrompt. 
\fi 

% We proposed a method, named Divide-and-Conquer Attack, which cleverly avoids semantic accuracy prompts and successfully jailbreaks the LLM-assisted Safety Filter. This method has found adversarial prompts in that space, demonstrating a security vulnerability.

==> sec/6_eval_setup.tex <==
% \section{Evaluation}

\if 0
We conduct evaluation to assess our proposed LLM-based adversarial prompt generation from multiple aspects. 
Revising the attack process in Equation~\ref{eq-attack_process}, the criteria for an effective adversarial prompt $T_a$ are twofold: first, its embedding vector must fall into the safe and logical area, as illustrated in Figure~\ref{fig-attack_modeling}(d) to bypass the safety filter; second, the image it generates should accurately capture the semantic intent expressed in the original drawing prompt $T$, as represented by the gray area in Figure~\ref{fig-attack_modeling}(d). Meeting both criteria is essential.

Therefore, in our evaluation, first, we aim to evaluate whether our attack can bypass the LLM-assisted safety filters of T2I models, which has not been effectively achieved by prior search-and-replace methods.
Secondly, we aim to evaluate the extent to which the images generated by our attack align with the attack intent expressed in the original drawing prompt.
Thirdly, since our attack leverages an LLM, we want to evaluate the cost induced by the attack to assess its potential security implications.
\fi 

% \begin{figure*}[t]
%     % \centering
%     % \includegraphics[width=0.98\linewidth]{figure/bypass_rate_dalle_onetime.jpg}
%     % \caption{\textcolor{red}{todo}}
%     % \label{fig:eval_bypass_dalle}
%     \centering
%     \begin{subfigure}{0.49\linewidth}
%         \includegraphics[width=\linewidth]{figure/bypass_rate_dalle_onetime.jpg}
%         \caption{Bypass rate of one-time attack.}
%         \label{fig:bypass_dalle_onetime}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}{0.49\linewidth}
%         \includegraphics[width=\linewidth]{figure/bypass_rate_dalle_reuse.jpg}
%         \caption{Bypass rate of reuse attack.}
%         \label{fig:bypass_dalle_reuse}
%     \end{subfigure}
%     \caption{Bypass rate of our attack across various LLM backbones.}
%     \label{fig:bypass_dalle}
% \end{figure*}

% \begin{figure*}[t]
%     % \centering
%     % \includegraphics[width=0.98\linewidth]{figure/bypass_rate_dalle_onetime.jpg}
%     % \caption{\textcolor{red}{todo}}
%     % \label{fig:eval_bypass_dalle}
%     \centering
%     \begin{subfigure}{0.47\linewidth}
%         \includegraphics[width=\linewidth]{figure/bypass_rate_midjourney_onetime.jpg}
%         \caption{Bypass rate of one-time attack.}
%         \label{fig:bypass_mid_one_time}
%     \end{subfigure}
%     % \hfill
%     \begin{subfigure}{0.47\linewidth}
%         \includegraphics[width=\linewidth]{figure/bypass_rate_midjourney_reuse.jpg}
%         \caption{Bypass rate of re-use attack.}
%         \label{fig:bypass_mid_reuse}
%     \end{subfigure}
%     \caption{Bypass rate of our attack across various T2I models}
%     \label{fig:bypass_mid}
% \end{figure*}


\renewcommand{\arraystretch}{1.30}
\begin{table*}[htbp]
  \caption{Bypass rate of our attack across various LLM backbones.}
  \centering
  \resizebox{\textwidth}{!}{%
  \begin{tabular}{ccccccccccccc}
    \toprule
    \textbf{Type} & \multicolumn{2}{c}{\textbf{Violence}} & \multicolumn{2}{c}{\textbf{Bloodiness}} & \multicolumn{2}{c}{\textbf{Crime}} & \multicolumn{2}{c}{\textbf{Discrimination}} & \multicolumn{2}{c}{\textbf{Eroticism}} & \multicolumn{2}{c}{\textbf{Mean}} \\
    \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9} \cmidrule(lr){10-11} \cmidrule(lr){12-13}
     & \textbf{One-time} & \textbf{Re-use} & \textbf{One-time} & \textbf{Re-use} & \textbf{One-time} & \textbf{Re-use} & \textbf{One-time} & \textbf{Re-use} & \textbf{One-time} & \textbf{Re-use} & \textbf{One-time} & \textbf{Re-use} \\
    \midrule
    GPT-4.0    & 86\%   & 85\%   & 65\%   & 80\%   & 92\%   & 90\%   & 87\%   & 85\%   & 44\%   & 75\%   & 74.8\% & 83\%   \\
    GPT-3.5    & 76\%   & 80\%   & 45\%   & 75\%   & 72\%   & 85\%   & 57\%   & 80\%   & 26\%   & 70\%   & 55.2\% & 78\%   \\
    Spark V3.0 & 73\%   & 95\%   & 57\%   & 100\%  & 78\%   & 100\%  & 63\%   & 100\%  & 35\%   & 85\%   & 61.2\% & 96\%   \\
    ChatGLM    & 91\%   & 95\%   & 65\%   & 100\%  & 67\%   & 100\%  & 87\%   & 95\%   & 36\%   & 80\%   & 69.2\% & 94\%   \\
    Qwen-14B   & 64\%   & 95\%   & 34\%   & 95\%   & 67\%   & 90\%   & 46\%   & 100\%  & 23\%   & 95\%   & 46.8\% & 95\%   \\
    Qwen-Max   & 96\%   & 100\%  & 73\%   & 100\%  & 87\%   & 100\%  & 82\%   & 100\%  & 45\%   & 90\%   & \textbf{76.6\%} & \textbf{98\%}  \\
    \bottomrule
  \end{tabular}
  }
  \label{tab:bypass_dalle}
\end{table*}


\renewcommand{\arraystretch}{1.30}
\begin{table*}[htbp]
  \caption{Bypass rate of our attack across various T2I models.}
  \centering
  \resizebox{\textwidth}{!}{%
  \begin{tabular}{ccccccccccccc}
    \toprule
    \textbf{Type} & \multicolumn{2}{c}{\textbf{Violence}} & \multicolumn{2}{c}{\textbf{Bloodiness}} & \multicolumn{2}{c}{\textbf{Crime}} & \multicolumn{2}{c}{\textbf{Discrimination}} & \multicolumn{2}{c}{\textbf{Eroticism}} & \multicolumn{2}{c}{\textbf{Mean}} \\
    \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9} \cmidrule(lr){10-11} \cmidrule(lr){12-13}
     & \textbf{One-time} & \textbf{Re-use} & \textbf{One-time} & \textbf{Re-use} & \textbf{One-time} & \textbf{Re-use} & \textbf{One-time} & \textbf{Re-use} & \textbf{One-time} & \textbf{Re-use} & \textbf{One-time} & \textbf{Re-use} \\
    \midrule
    \dalle~3    & 86\%   & 85\%   & 65\%   & 80\%   & 92\%   & 90\%   & 87\%   & 85\%   & 44\%   & 75\%   & 74.8\% & 83\%   \\
    Midjourney V6    & 80\%   & 90\%   & 60\%   & 80\%   & 60\%   & 80\%   & 80\%   & 90\%   & 40\%   & 80\%   & 64.0\% & 84\%   \\
    \bottomrule
  \end{tabular}
  }
  \label{tab:bypass_mid}
\end{table*}

\if 0
\subsection{Evaluation Settings}
\label{sec-eval-setting}

Driven by above evaluation goals, we adopt the following evaluation settings:

\textbf{Targeted T2I models}. We adopt two state-of-the-art T2I models, \dalle~3~\cite{dalle3} and Midjourney V6~\cite{midjourney} equipped with LLM-asssited safety filter as the victims of our attack. 
They offer two access modes: an online interactive interface and API mode. 
In API mode, it accepts the prompt at once and generates images, or it may reject the prompt if its safety filter detects sensitive content. 

We have noted that there are some text-based safety filters in the open-source community, such as the NSFW text matching filter~\cite{george2020nsfw}, which blocks harmful content by identifying keywords from a predefined NSFW dictionary. Another example is the NSFW text classifier from Huggingface~\cite{li2022nsfw}, which fine-tunes DistilBERT~\cite{sanh2019distilbert} with text from an NSFW channel on Reddit for NSFW/SFW classification~\cite{nsfwgpt2023}. However, through experimentation, we observed that these open-source filters are less effective across a broader range of topics, such as VBCDE-100, and they fail most of the time to detect the adversarial prompts generated by DACA. Therefore, in the following section, we primarily use API of \dalle~3 and Midjourney for evaluation.
\fi 

% In the online interactive interface, the model maintains a context window, allowing the attacker to input adversarial prompts sentence by sentence and observe the generated image at each step. We also utilize it to intuitively demonstrate our attack effect.

% \textbf{LLM(s) Backbone used by the Attacker}. 
% Our attack leverages LLMs for adversarial prompt generation. To evaluate the impact of LLM capacity, we selected 6 LLMs based on existing evaluation results from public benchmarks such as SuperCLUE~\cite{superclueai}, Chatbot Arena~\cite{arena}, and Open Compass~\cite{opencompass}. Our chosen LLMs are GPT-4\cite{openai_pricing}, GPT-3.5-turbo\cite{openai_pricing}, Spark V3.0\cite{spark_pricing}, ChatGLM-turbo\cite{chatglm_pricing}, Qwen-14B\cite{qianwen_14_pricing}, and Qwen-Max\cite{qianwen_max_pricing}. We utilize their API mode for large-scale, automated assessment and comparison, with API pricing scheme as shown in Table~\ref{tab:llm_pricing}. 

% \begin{table}[t]
% \caption{API pricing schemes, \ie, the cost per 1,000 tokens for LLM backbone in our evaluation.}
% \centering
% \resizebox{\linewidth}{!}{%
% \begin{tabular}{|c|c|c|c|}
% \hline
% Models & Input Token (\$) & Output Token (\$) & Words/Tokens \\ \hline
% GPT-4.0~\cite{openai_pricing} & 0.003  & 0.006 & 0.75 \\ \hline
% GPT-3.5-turbo~\cite{openai_pricing} & 0.001 & 0.002  & 0.75 \\ \hline
% Spark V3.0~\cite{spark_pricing} & 0.005 & 0.005 & 0.8 \\ \hline
% ChatGLM-turbo~\cite{chatglm_pricing} & 0.0007 & 0.0007 & 0.56 \\ \hline
% Qwen-14B~\cite{qianwen_14_pricing}  & 0.001  & 0.001 & 1  \\ \hline
% Qwen-Max~\cite{qianwen_max_pricing} & free for now & free for now & 1  \\ \hline
% \end{tabular}%
% }
% \label{tab:llm_pricing}
% \end{table}

\begin{table}[t]
\caption{API pricing schemes, \ie, the cost per 1,000 tokens for LLM backbones in our evaluation.}
\centering
\resizebox{\linewidth}{!}{%
\begin{tabular}{lccc}
\toprule
\textbf{Models} & \textbf{Input Token (\$)} & \textbf{Output Token (\$)} & \textbf{Words/Tokens} \\
\midrule
GPT-4.0~\cite{openai_pricing} & 0.003  & 0.006 & 0.75 \\
GPT-3.5-turbo~\cite{openai_pricing} & 0.001 & 0.002  & 0.75 \\
Spark V3.0~\cite{spark_pricing} & 0.005 & 0.005 & 0.8 \\
ChatGLM-turbo~\cite{chatglm_pricing} & 0.0007 & 0.0007 & 0.56 \\
Qwen-14B~\cite{qianwen_14_pricing}  & 0.001  & 0.001 & 1  \\
Qwen-Max~\cite{qianwen_max_pricing} & \multicolumn{2}{c}{free for now} & 1  \\
\bottomrule
\end{tabular}%
}
\label{tab:llm_pricing}
\end{table}


\if 0
\textbf{Targeted Drawing Prompt Set}. 
In our evaluation, the content scope of the targeted drawing prompt set extends beyond the NotSafeForWork (NSFW) content studied in prior works~\cite{yang2023sneakyprompt, ba2023surrogateprompt}, which primarily focused on inappropriate sexual content. According to content moderation guidelines specified by T2I models~\cite{midjourney-ban, dalle_systemcard}, harmful content also includes categories such as gore, violence, discrimination, \etc.
Thus, we curated a diverse drawing prompt dataset called the VBCDE-100 (\textbf{V}iolent-\textbf{B}loody-\textbf{C}rime-\textbf{D}iscriminate-\textbf{E}rotic) dataset, which includes 100 sensitive prompts across five categories: violence, gore, illegal activities, discrimination, and pornographic content. Each category is represented by approximately 20 sensitive prompts, ensuring broad coverage of the potential censorship range enforced by T2I models.
% Additionally, considering the copyright restrictions integrated into T2I models for protecting intellectual property, we have also developed a dataset focusing on copyright issues, called Copyright-20 dataset, including 10 prompts about Copyright Characters and 10 about artists' styles protected under copyright laws post-1912. 
Our empirical testing confirmed that all sensitive prompts were consistently rejected by the safety filters of our targeted T2I models for image generation, validating the relevance of our dataset. 
This dataset can also serve future research by enabling the exploration of T2I model safety filters. 
% contributing to a deeper understanding of how these models defend against sensitive content. 
\fi 

% \section{Evaluation Setup}
% \subsection{Victim TTI Models}

% We adopt two SOTA TTI models, \dalle~3~\cite{dalle3} and Midjourney V6~\cite{midjourney} as the victim of our attack. 
% They offer two access modes: an online interactive interface and API mode. 
% In the API mode, it accepts the prompt at once and generates images, or it may reject the prompt if its safety filter detects sensitive content. We mainly use API for evaluation. 
% In the online interactive interface, the model maintains a context window, allowing the attacker to input adversarial prompts sentence by sentence and observe the generated image at each step. We also utilize it to intuitively demonstrate our attack effect.

% \subsection{LLM(s) Backbone as Attack Assistants}

% Our attack leverages LLMs as the assitants for adversarial prompt generation. 
% Thus, we choose 6 LLMs with different capacities for evaluation: \texttt{GPT-4}~\cite{openai_pricing}, \texttt{GPT-3.5-turbo}~\cite{openai_pricing}, \texttt{Spark V3.0}~\cite{spark_pricing}, \texttt{ChatGLM-turbo}~\cite{chatglm_pricing}, \texttt{Qwen-14B}~\cite{qianwen_14_pricing}, and \texttt{Qwen-Max}~\cite{qianwen_max_pricing}.
% Based on the ranking from various public benchmarks such as SuperCLUE~\cite{superclueai}, Chatbot Arena~\cite{arena}, and Open Compass~\cite{opencompass}, the approximate descending order of model capability is: GPT-4.0, Qwen-max, GPT-3.5-turbo, ChatGLM-turbo, SparkV3.0 Qwen-14B.
% We utilize the API mode of LLMs for large-scale, automated assessment and comparison.



% \subsection{Attack Topic}
% In our jailbreak research on the LLM-assisted Safety Filter for TTI engines, we adopt a broader perspective to define and identify harmful content. Previous studies primarily focused on inappropriate sexual content (NSFW), but harmful content extends far beyond this. According to content moderation standards from companies like OpenAI and Meta, harmful content also includes categories like gore, violence, discrimination, and political sensitivity. These types of content can potentially harm users and thus must be strictly monitored and filtered.

% Moreover, as AI technology becomes more widespread and mature, the protection of copyrights in artistic works is increasingly emphasized by many institutions. For example, OpenAI's DALL-E 3 TTI engine takes special note of copyright protection, refusing to generate reproductions of artworks created by artists after 1923. This reflects an important trend, where AI technology needs to find a balance between innovation and copyright law.

% Therefore, our research not only focuses on traditional harmful content but also extends to copyrighted materials. Through this approach, we aim to comprehensively assess and test the effectiveness and limitations of TTI engine safety filters when facing diverse and complex harmful content. We explore different types of adversarial prompts, analyze how they bypass filtering mechanisms, and examine the possibilities of generating such content without triggering safety alarms.

% \subsection{Unethical Prompt Dataset}

% Most current attempts to circumvent TTI models~\cite{yang2023sneakyprompt, ba2023surrogateprompt}, predominantly target Not Safe For Work (NSFW) content, especially pornographic images. However, based on official documentation and our own empirical analyses of the latest TTI models, including DALL·E 3 and MidJourney, it is observed that their safety filters extend well beyond just NSFW content. These models will decline requests related to a wide array of topics, including violence, gore, illegal activities, discrimination, and pornography. 

% Consequently, datasets on NSFW content~\cite{yang2023sneakyprompt} may not provide a comprehensive basis for assessing the capability to bypass the safety filters of SOTA TTI models.

% Thus, we curate a diverse dataset called the VBCDE-100 dataset, which including 100 sensitive prompts spread across five categories: violence, gore, illegal activities, discrimination, and pornographic content. 
% Each category is represented by approximately 20 sensitive prompts, ensuring a broad coverage of the potential censorship range implemented by various TTI models. 
% Additionally, considering the copyright restrictions integrated into TTI models for protecting intellectual property, we have also developed a dataset focusing on copyright issues, called Copyright-20 dataset, including 10 prompts about Copyright Characters and 10 about artists' styles protected under copyright laws post-1912. 
% Our empirical testing confirmed that all these sensitive prompts were consistently rejected by the SOTA models for image generation, validating the relevance and utility of our dataset.
% We hope our dataset can aid future research in exploring the safety filters of T2I models, contributing to deeper understanding of how these models manage sensitive and copyrighted content.



% \subsection{Evaluation Methodology}

% Our attack objective is outlined as follows: For an unethical prompt \(p_s\) that is detected and blocked by the safety filter (\(\mathcal{F}(\mathcal{M}, p_s) = 1\)), our goal is to develop a prompt transformation approach \(\mathcal{T}\). This method is intended to produce an adversarial prompt \(p_{adv} = \mathcal{T}(p_s)\) such that \(\mathcal{F}(\mathcal{M}, p_{adv}) = 0\) and the resulting image \(\mathcal{M}(p_{adv})\) closely resembles the visual semantics of \(\mathcal{M}(p_s)\).
% It is important to note that the concept of adversarial prompt is relative, as highlighted in~\cite{yang2023sneakyprompt}. The adversarial nature of \(p_{adv}\) is specifically in comparison to the unethical prompt \(p_s\), which is initially blocked by the safety filter \(\mathcal{F}\). 
% The criteria for an effective adversarial prompt \(p_{adv}\) are twofold: firstly, it must circumvent the safety filter \(\mathcal{F}\), and secondly, the image it generates should accurately reflect the intent expressed in \(p_s\). Fulfilling both criteria is crucial. 

% \textbf{Evaluation Methodology}.
% For each sensitive drawing prompt within VBCDE-100, we employ 6 LLMs to generate its adversarial prompts, producing between 5 to 10 adversarial prompts per LLM. This process yields a total of 50-100 adversarial prompts for each sensitive prompt, and \textbf{3600} adversarial prompts for image generation in total. 

\if 0
We consider two attack cases in our evaluation:

\noindent$\bullet$ One-time attack: For each prompt $T$, the adversary generate its corresponding adversarial prompt $T_a$ for a single use. Each time, a new adversarial prompt can be obtained by invoking the LLM-based prompt generation method (Equation~\ref{eq-attack_process}) again. 

\noindent$\bullet$ Re-use attack: The adversary utilizes adversarial prompts $T_a$ generated in previous one-time attacks and reuses them, \ie, inputs them into the T2I model for generating more unethical images. This scenario implies that the generated prompts can be stored for future use, thereby extending their impact.


% For Copyright-20 dataset, we employ a methodology akin to that used for VBCDE-100, generating 10 adversarial prompts for each sensitive prompt using a LLM, leading to a total of 60 prompts per sensitive prompt. This approach results in the creation of \textbf{1200} adversarial prompts in total.

% \(20 \times 6 \times 10 = \textbf{1200}\) 
\underline{\dalle~3 as the victim:}
In "one-time attack" evaluation, all adversarial prompts are individually input into \dalle~3 for image generation. To evaluate the success of "re-use attack", we select several adversarial prompts from each combination of sensitive category and LLM, specifically choosing those whose resultant images most closely align with the original drawing prompt in terms of semantic coherence. Each chosen prompt is then used to generate images via \dalle~3 an additional 10 times. For VBCDE-100 dataset, we have \textbf{1800} reuse attack instances against \dalle~3.
% For Copyright-20 dataset, we obtain \(20 \times 6 \times 10 = \textbf{1200}\) images to evaluate the effectiveness of the reuse attack.

% For each sensitive prompt in the VBCDE-100 dataset, we transform it using 6 different Large Language Model (LLM) backbones, generating 5 to 10 adversarial prompts per LLM, thus resulting in 50-100 adversarial prompts per sensitive prompt. The VBCDE-100 dataset altogether generates \textbf{3600} adversarial prompts. In the context of a one-time attack evaluation, we feed these prompts individually into \dalle~3 to generate images. To assess the effectiveness of the reuse attack, we select multiple adversarial prompts for each combination of sensitive category and LLM backbone. Specifically, we choose the prompts whose generated images maintain the highest semantic coherence with the original sensitive prompt. Then, each selected prompt is fed into \dalle~3 to generate images 10 additional times, resulting in \textbf{1800} reuse attack trials against \dalle~3.

\underline{Midjourney V6 as the victim:}
% Midjourney V6 has little restriction on copyright, thus we only evaluate it on VBCDE-100.
From 5 categories of adversarial prompts generated by GPT-4 for the VBCDE-100 dataset, we select 5 prompts from each category. 
% These selected prompts are ones that would be blocked by MidJourney's safety filter if the original sensitive prompts were used. 
Through the Discord Interface~\cite{discord} of MidJourney, inputting a single prompt results in the generation of 4 images; thus, for our "one-time attack" evaluation, we generate a total of \(25 \times 4 = 100\) images.
Subsequently, we identify the 5 prompts that yielded images with the greatest semantic coherence to the original sensitive prompts. Reusing these 5 prompts to generate images with MidJourney 10 additional times produces \(10 \times 5 \times 4 = 200\) images to evaluate the "re-use attack". 
% Given considerations of cost and time, we limit our experiments with MidJourney to using GPT-4 as the sole LLM backbone.

\fi 

==> sec/7_eval.tex <==
% \section{Evalution}
% 我们要证明什么？
% 1.成功bypass
% Bypass这里说明一下，开源过滤器也能够成功通过。

% 2.成功expose
% 3.攻击开销如何
% 我们用三个问题来揭示

% Our evaluation is designed to address the following research questions (RQs):

% \noindent$\bullet$ [RQ1] How effective is our attack in bypassing the safety filters of SOTA TTI models?\\
% \noindent$\bullet$ [RQ2] How is the semantic coherence of image generated under our attack?\\
% \noindent$\bullet$ [RQ3] What is the cost-effectiveness of our attack?


\subsection{Eval@Bypassing Filter Effectiveness}


% \noindent\textbf{Evaluation Metrics}. 
In this part, we adopt the bypass rate as the evaluation metric. 
For the one-time attack, we compute the bypass rate as the ratio of adversarial prompts that successfully circumvent the safety filter to the total number of adversarial prompts. For the re-use attack, the bypass rate is calculated as the proportion of reuse attempts that bypass safety filter. 
 
\noindent\textbf{Bypass rate@\dalle~3.} 
The success rates of the DACA in bypassing \dalle~3's safety filter are shown in Figure~\ref{fig:bypass_dalle}. 
We separately calculated the bypass rate for one-time attack and re-use attack across 6 different backbone LLMs.
% \underline{Bypass rate@VBCDE-100}. 
As illustrated in Figure~\ref{fig:bypass_dalle}, our attack against \dalle~3 exhibits good performance on the VBCDE-100 dataset. During the one-time attack, DACA achieved a considerably high average success rate of \textbf{80.4\%} across different LLMs and topics. In the re-use attack, DACA demonstrates great stability, maintaining a high reuse bypass success rate across all topics, with the Qwen-Max model achieving an average reuse success rate of \textbf{98.0\%} across its five topics. According to the system card~\cite{dalle_systemcard} of  \dalle~3, OpenAI team has made extra efforts to restrict sex-related content. Therefore, it is expected that the success rate for the eroticism topic would be lower than that of other topics during the one-time bypass tests. As shown on Figure~\ref{fig:bypass_dalle_reuse}, once bypassed the strict restriction over eroticism, the adversarial prompts can also exhibits a high reuse bypass success rate.

% \underline{Bypass rate@Copyright-20.} 
% According to Table \ref{tab:copyright}, We observed that copyright-protected content showed a high bypass success rate for both one-time and re-use attack. 

\if 0
\renewcommand{\arraystretch}{1.0}
\begin{table*}[ht]
\centering
\caption{Bypass Rate of our attack(Target:\dalle~3)}
\resizebox{\linewidth}{!}{%
\begin{tabular}{|c|cc|cc|cc|cc|cc|cc|}
\hline
\textbf{Backbone LLMs} & \multicolumn{2}{c|}{\textbf{GPT-4.0}}  & \multicolumn{2}{c|}{\textbf{GPT-3.5-turbo}} & \multicolumn{2}{c|}{\textbf{Spark V3.0}} & \multicolumn{2}{c|}{\textbf{ChatGLM-turbo}} & \multicolumn{2}{c|}{\textbf{Qwen-14B}} & \multicolumn{2}{c|}{\textbf{Qwen-Max}} \\ \hline
Categories             & \multicolumn{1}{c|}{One-time} & Re-use & \multicolumn{1}{c|}{One-time}    & Re-use   & \multicolumn{1}{c|}{One-time}  & Re-use  & \multicolumn{1}{c|}{One-time}    & Re-use   & \multicolumn{1}{c|}{One-time} & Re-use & \multicolumn{1}{c|}{One-time} & Re-use \\ \hline
Copyright Character    & \multicolumn{1}{c|}{98\%}     & 99\%   & \multicolumn{1}{c|}{96\%}        & 100\%    & \multicolumn{1}{c|}{96\%}      & 78\%    & \multicolumn{1}{c|}{97\%}        & 97.5\%   & \multicolumn{1}{c|}{90\%}     & 94\%   & \multicolumn{1}{c|}{76\%}     & 100\%  \\ \hline
Artists'Style          & \multicolumn{1}{c|}{98\%}     & 96\%   & \multicolumn{1}{c|}{95\%}        & 80\%     & \multicolumn{1}{c|}{80\%}      & 85\%    & \multicolumn{1}{c|}{83\%}        & 78\%     & \multicolumn{1}{c|}{80\%}     & 85\%   & \multicolumn{1}{c|}{89\%}     & 86\%   \\ \hline
\end{tabular}
}
\label{tab:copyright}
\end{table*}
\fi 

\noindent\textbf{Bypass Rate@Midjourney V6.} 
As illustrated in Figure~\ref{fig:bypass_mid_one_time}, the one-time bypass rate for Midjourney is marginally lower than that of \dalle~3. This difference can be attributed to Midjourney's safety filter, which reject potentially bad requests during the initial word filtering stage~\cite{midjourney-ban}. However, once a text manages to circumvent Midjourney's initial safety detection, the probability of successfully bypassing the system in subsequent attempts increases, as indicated by its higher reuse bypass rate in comparison to \dalle~3 in Figure~\ref{fig:bypass_mid_reuse}. 

\begin{mdframed}[style=MyFrame,nobreak=false,align=left, userdefinedwidth=\linewidth]
        \textbf{[Key Takeaway]}: The LLM-based method, DACA, can successfully rephrase prompts to generate adversarial versions that bypass the advanced LLM-assisted safety filters of \dalle~3 and the Midjourney model with a high success rate, even when using a relatively small 14B LLM model as the backbone.
\end{mdframed}


\subsection{Eval@Image Generation Precision}
\label{sec-eval-image-review}
% \noindent\textbf{Evaluation Metric for Semantic Similarity}. 
To evaluate the semantic similarity/matching degree between the images generated by our attacks and the original drawing prompts, we employ both objective (by quantitative metric or algorithm) and subjective (by human) assessments.
% covering three types of assessment methods.

% To assess the semantic similarity between the generated images and the original sensitive prompt, we evaluate from both subjective manual review and also objective algorithm accesss, CLIP-based embedding similarity an also GPT-4 image analysis. 

\subsubsection{CLIP-embeddings-based Image Assessment}
% \noindent\underline{CLIP Model Embeddings~\cite{clip_repo}}: 
Similar to prior research~\cite{shan2023promptspecific, yang2023sneakyprompt}, we utilize the pre-trained CLIP model encoder~\cite{clip_repo} to derive text and image embeddings for similarity calculations. CLIP, trained on a vast dataset of images paired with their textual descriptions, aligns texts and images within a unified dimensional space, thereby effectively capturing the semantic similarities across these two modalities.

Our application of CLIP embeddings is twofold:

\textbf{Text-Image Similarity}: We assess the cosine similarity~\cite{rahutomo2012semantic} between the CLIP embeddings of the generated images and the sensitive prompts. This evaluates the semantic coherence, \ie, how well the generated images reflect the intended concepts of the original prompts.
To apply text-image similarity, we initiated a procedure to determine a reference. Specifically, we curated a set of 100 prompts, ensuring that each prompt would result in image generation without being blocked. Then we utilized the CLIP model's encoder to analyze the embeddings of these text-image pairs. Through this analysis, we calculated the cosine similarity for each pair, leading to an average of 0.274 across the 100 pairs, as indicated by orange horizontal line in Figure~\ref{fig:clip_score}. This serves as an indicative measure of the model's capability to accurately translate textual descriptions into coherent visual representations. We employ it as a reference to assess the quality our approach on generating images from adversarial prompts, \ie, higher or equal to it can be regarded as satisfying. As depicted in Figure~\ref{fig:clip_score}, the cosine similarity scores of CLIP embeddings for all images produced during the reuse attack and their respective original sensitive prompts, closely align with the reference value (as indicated by the solid orange line). This suggests that the images generated through our attack maintain satisfying semantic coherence with the original sensitive prompts.

\textbf{Text-Text Similarity}: We compute the cosine similarity between the CLIP embeddings of the adversarial prompts and their corresponding sensitive prompts to quantify the extent to which the semantic integrity of the original prompt is retained within our adversarial prompts. 
It's important to note that the reference value for text-text similarity is typically higher than that for text-image one, primarily due to the uniformity of modality in text-text comparisons.
Figure~\ref{fig:clip_score} shows the high cosine similarity scores observed between the adversarial prompts and the original sensitive prompts. 
Despite the modifications made to the original prompts, the essence of the prompts remain largely intact.
However, these semantically similar adversarial prompts did not activate the safety filters of T2I models during our evaluations. 
This highlights the need to strengthen the security measures of T2I models.

\begin{figure}[t]
    \centering
    \includegraphics[width=0.95\linewidth]{figure/similarity_dalle_reuse_clip.jpg}
    \caption{CLIP-embeddings-based Image Assessment.}
    \label{fig:clip_score}
\end{figure}

% \begin{figure}[ht]
%     \centering
%     \includegraphics[width=0.95\linewidth]{figure/similarity_dalle_reuse_gpt4_review.jpg}
%     \caption{GPT-4 Review (Target: \dalle~3)}
%     \label{fig:gpt-4}
% \end{figure}


% \begin{figure}[ht]
%     \centering
%     \includegraphics[width=0.95\linewidth]{figure/similarity_midjourney_reuse_gpt4_review.jpg}
%     \caption{GPT-4 Review (\dalle~3 v.s. Midjourney)}
%     \label{fig:mid_gpt4}
% \end{figure}

% \begin{figure*}[ht]
%     \centering
%     \begin{subfigure}{0.49\linewidth}
%         \includegraphics[width=\linewidth]{figure/similarity_dalle_reuse_gpt4_review.jpg}
%         \caption{Across various LLM backbone}
%         \label{fig:gpt-4}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}{0.48\linewidth}
%         \includegraphics[width=\linewidth]{figure/similarity_midjourney_reuse_gpt4_review.jpg}
%         \caption{Across various T2I Models: \dalle~3 v.s. Midjourney}
%         \label{fig:mid_gpt4}
%     \end{subfigure}
%     \caption{Evaluation results of GPT-4-based Image Assessment.}
%     \label{fig-gpt4-review}
% \end{figure*}

% \begin{figure*}[ht]
%     \centering
%     \begin{subfigure}{0.49\linewidth}
%         \includegraphics[width=\linewidth]{figure/similarity_dalle_reuse_manual_1.jpg}
%         \caption{Results of Task I.}
%         \label{fig:manual_1}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}{0.49\linewidth}
%         \includegraphics[width=\linewidth]{figure/similarity_dalle_reuse_manual_2.jpg}
%         \caption{Results of Task II.}
%         \label{fig:manual_2}
%     \end{subfigure}
%     \caption{Evaluation results of Manual Image Assessment.}
%     \label{fig-manual}
% \end{figure*}


\begin{table}[htbp]
  \centering
  \caption{\dalle~3 Evaluation results of GPT-4-based Image Assessment.}
  \resizebox{\linewidth}{!}{%
  \begin{tabular}{cccccc}
    \toprule
    \textbf{Type} & \textbf{Violence} & \textbf{Bloodiness} & \textbf{Crime} & \textbf{Discrimination} & \textbf{Eroticism} \\
    \midrule
    GPT-4.0    & 60\%  & 30\% & 55\% & 50\% & 5\%   \\
    GPT-3.5    & 45\%  & 25\% & 50\% & 45\% & 0\%   \\
    Spark V3.0 & 55\%  & 30\% & 50\% & 50\% & 5\%   \\
    ChatGLM    & 45\%  & 20\% & 60\% & 55\% & 5\%   \\
    Qwen-14B   & 45\%  & 15\% & 45\% & 40\% & 5\%   \\
    Qwen-Max   & 65\%  & 35\% & 60\% & 50\% & 10\%  \\
    \bottomrule
  \end{tabular}
}
  \label{tab:similarity_dalle_reuse_gpt4_review}
\end{table}

\begin{table}[htbp]
  \centering
  \caption{\dalle~3 Evaluation results of GPT-4-based Image Assessment compared with Midjourney V6.}
  \resizebox{\linewidth}{!}{%
  \begin{tabular}{cccccc}
    \toprule
    \textbf{Type} & \textbf{Violence} & \textbf{Bloodiness} & \textbf{Crime} & \textbf{Discrimination} & \textbf{Eroticism} \\
    \midrule
    \dalle~3    & 60\%  & 30\% & 55\% & 50\% & 5\%   \\
    Midjourney V6    & 37\%  & 27\% & 40\% & 25\% & 0\%   \\
    \bottomrule
  \end{tabular}
}
  \label{tab:similarity_midjourney_reuse_gpt4_review}
\end{table}



\renewcommand{\arraystretch}{1.30}
\begin{table*}[htbp]
  \centering
  \caption{Evaluation results of Manual Image Assessment.}
  \resizebox{\textwidth}{!}{%
  \begin{tabular}{ccccccccccccc}
    \toprule
    \multirow{2}{*}{\textbf{Type}} & \multicolumn{2}{c}{\textbf{Violence}} & \multicolumn{2}{c}{\textbf{Bloodiness}} & \multicolumn{2}{c}{\textbf{Crime}} & \multicolumn{2}{c}{\textbf{Discrimination}} & \multicolumn{2}{c}{\textbf{Eroticism}} & \multicolumn{2}{c}{\textbf{Mean}} \\
    \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9} \cmidrule(lr){10-11} \cmidrule(lr){12-13}
     & \textbf{Task I} & \textbf{Task II} & \textbf{Task I} & \textbf{Task II} & \textbf{Task I} & \textbf{Task II} & \textbf{Task I} & \textbf{Task II} & \textbf{Task I} & \textbf{Task II} & \textbf{Task I} & \textbf{Task II} \\
    \midrule
    GPT-4.0    & 2.7  & 59.0\%  & 1.3  & 25.0\%  & 3.0  & 53.5\%  & 2.6  & 48.5\%  & 0.2  & 5.0\%   & 2.0  & 38.2\%  \\
    GPT-3.5    & 2.6  & 52.0\%  & 1.2  & 23.0\%  & 2.9  & 50.0\%  & 2.5  & 47.0\%  & 0.1  & 3.0\%   & 1.9  & 35.0\%  \\
    Spark V3.0 & 2.8  & 57.5\%  & 1.3  & 23.0\%  & 2.9  & 51.0\%  & 2.5  & 47.5\%  & 0.2  & 4.0\%   & 1.9  & 36.6\%  \\
    ChatGLM    & 2.6  & 58.5\%  & 1.3  & 23.5\%  & 2.8  & 50.0\%  & 2.6  & 49.0\%  & 0.1  & 4.0\%   & 1.9  & 37.0\%  \\
    Qwen-14B   & 2.4  & 49.0\%  & 1.1  & 20.0\%  & 2.5  & 53.5\%  & 2.4  & 37.5\%  & 0.0  & 2.0\%   & 1.7  & 32.4\%  \\
    Qwen-Max   & 3.0  & 61.0\%  & 1.3  & 25.5\%  & 3.1  & 54.5\%  & 2.7  & 49.0\%  & 0.1  & 4.0\%   & 2.0  & 38.8\%  \\
    Mean       & 2.7  & 56.0\%  & 1.3  & 23.3\%  & 2.9  & 52.1\%  & 2.6  & 46.4\%  & 0.1  & 3.7\%   & /    & /     \\
    \bottomrule
  \end{tabular}
  }
  \label{tab:similarity_dalle_reuse_manual}
\end{table*}

% The overall results are shown in Figure~\ref{fig:clip_score},\ref{fig:manual_1},\ref{fig:manual_2},\ref{fig:gpt-4}. 

% \noindent\underline{GPT-4 Image Review}: 

\subsubsection{GPT-4-based Image Assessment}
\label{sec-gpt4-assess}
Considering that existing LLMs also feature image understanding capabilities, we utilized GPT-4 to evaluate the content of the generated images. Specifically, we input the generated images into ChatGPT, instructing it to analyze the images and determine whether they contain certain sensitive content. We employ the following prompt:

\begin{mdframed}[style=MyFrame,nobreak=false,align=left, userdefinedwidth=\linewidth]
        \textbf{Prompt for GPT-4 Image Assessment:} \\
        What's in this image? Is this image suitable for exhibition? \\
        Please answer in the following format: \\
        {[Appropriate/Inappropriate][Reason]}
\end{mdframed}


For all the images, we calculated the percentage deemed "inappropriate" by GPT-4 and present the results in Figure~\ref{fig-gpt4-review}. For violence, crime, and discrimination, more than half of the images generated by our adversarial prompts are detected as harmful by GPT-4, as shown in Figure~\ref{fig:gpt-4}. This suggests the potential for leveraging the image understanding capabilities of models like GPT-4 to implement post-generation filters, which will be further discussed in \S~\ref{sec-post-detect}.
% Our findings indicate that GPT-4 is more aggressive than manual checking in defining sensitivity. 
% As shown in Figure~\ref{fig:gpt-4}, more than half of the image generated by \dalle~3 under adversarial prompts are identified as harmful by GPT-4. 
As shown in Figure~\ref{fig:mid_gpt4}, fewer images generated by Midjourney were deemed harmful by GPT-4, compared to those from \dalle3. Based on our analysis, this can be attributed to Midjourney's relatively weaker capability in understanding and rendering prompts. Consequently, it may not accurately depict every aspect of the adversarial prompt with the same high quality as \dalle~3.
Some generated images can be be viewed in our Github repo.
% \footnote{https://github.com/researchcode001/Divide-and-Conquer-Attack}.

% Although Midjourney has a relatively high bypass success rate, its deficiency in prompt semantic understanding limits its ability to effectively express the harmful information contained in adversarial prompts, resulting in a lower review score.
% In terms of Copyright-20 dataset, it is found that the probability of being harmful for Copyright Character was significantly higher than for Artists’ Style. This is because copyright characters often possess uniqueness, making them easier to be described by "Divide", whereas describing artists' style presents more challenges. GPT-4's review of artist styles also finds it more difficult to distinguish styles. 


\subsubsection{Manual Image Assessment}
% \noindent\underline{Manual Review}: 
We then engaged 10 volunteers, varying in age, gender, and educational background, to assess the images generated through our attack. We provide guidance to the volunteers as shown in Appendix~\ref{sec-user-guidance}. We design two tasks: 

\textbf{Task 1}: Each volunteer is presented with a pair of a generated image and its original sensitive prompt, they were asked to rate the similarity between their content. The rating scale ranged from 1 to 5, where 1 signified minimal relevance and 5 denoted strong relevance. 
% This assessment aimed to evaluate the semantic alteration applied by our method to the original sensitive prompt.

\textbf{Task 2}: Given an image, participants should determine the ethical nature of its content and then categorize it as either “harmful” or “harmless”.
% mimicing what we ask GPT-4 to do in \S~\ref{}. 
% This is to evaluate DACA's ability to render the harmful semantic content. 


\begin{figure*}[ht]
    \centering
    \begin{subfigure}{0.48\linewidth}
        \includegraphics[width=\linewidth]{figure/cost_onetime_token.jpg}
        \caption{token usage.}
        \label{fig:cost_token}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.48\linewidth}
        \includegraphics[width=\linewidth]{figure/cost_onetime_money.jpg}
        \caption{money expense.}
        \label{fig:cost_money}
    \end{subfigure}
    \caption{Cost Effectiveness Evaluation.}
\end{figure*}

Based on the results shown in Figure~\ref{fig-manual}, volunteers generally rated the precision of images related to violence, crime, and discrimination as higher in quality compared to those depicting bloodiness and eroticism. 
Bloodiness and content generation are less satisfying, since the quantity of generated images with these harmful content is considerably lower compared to other categories in Figure~\ref{fig:manual_2}. Upon further examination, the challenge lies in that the sensitive elements being predominantly focused on details like blood, requiring finer-grained "Divide" strategy than our current implementation. We further discuss the effective generalization to various topics in \S~\ref{sec-generalize}.

\subsubsection{Distinction between Image Assessment Methods}
% CLIP-embedding-based, GPT-4-based, and manual evaluations. 
CLIP embeddings and cosine similarity calculations are widely used in related research~\cite{yang2023sneakyprompt, ba2023surrogateprompt} to provide semantic quantification across text and image modalities. However, whether CLIP-based embeddings fully reflect similarity as perceived by the human remains an open question. It is also unclear if there are better objective metrics than CLIP-based embeddings for capturing the nuanced semantic alignment between text and images. Thus, it seems that CLIP-based similarity is currently our best available choice for objective assessment. 
GPT-4-based method relies on the image understanding capabilities of the underlying multi-modal LLM, a technique that is continuously evolving. As LLMs improve, their ability to accurately interpret and assess images in relation to text is expected to become more refined, potentially offering more reliable evaluations in the future. 
Manual review by humans seems to provide the most reliable reference, but it is significantly impacted by user diversity and subjectivity, and also difficult to scale. 

Despite the absence of an optimal image evaluation metric, \textbf{we use multiple aspects to demonstrate that the proposed attack can indeed generate effective adversarial prompts to bypass LLM-assisted safety filters and also have non-negligible chances to obtain the intended harmful image, outperforming previous search-and-replace methods~\cite{yang2023sneakyprompt} that can not bypass LLM-assisted safety filters.}

% For Task II, around 50\% of the images were classified as harmful, indicating that half of the generated images retained harmful semantics. 
% This points to significant security implications.
% Besides the strictly controlled erotic content, bloodiness content generation is less satisfying, since the quantity of successfully generated images with harmful bloodiness content is considerably lower compared to other categories in Figure~\ref{fig:manual_2}. Upon further examination, the challenge lies in that the sensitive elements being predominantly focused on bloodiness itself, offering limited alternative sensitive elements for the "Divide" strategy to leverage. 

% Upon further examination, it appears that the challenge with bloodiness content lies in its sensitive elements being predominantly focused on the aspect of bloodiness itself, offering limited alternative sensitive elements for the "Divide" strategy to leverage. Consequently, the adversarial prompts processed through DACA retained less harmful information, rendering it more difficult to generate images that accurately reflect the original prompts' intent. This phenomenon is also evident in Figure~\ref{fig:manual_2}, where the quantity of successfully generated images with harmful bloodiness content is considerably lower compared to other categories, attributed to the substantial loss of harmful information.


% indicating a balanced distribution of images generated from the reuse attack in terms of their alignment with the original semantics. 
% From the data presented in Figure~\ref{fig:manual_2}, it can be inferred that approximately 50\% of the images remain aligned to the semantics of the initial sensitive prompts. 
% The manual evaluation of the reuse attack suggests that half of the generated images retained the harmful semantics, which implies non-negligible security implication.


% Figure~\ref{fig:manual_1} reveals that most scores hover between 2.5 to 3, indicating a balanced distribution of images generated from the reuse attack in terms of their alignment with the original semantics. From the data presented in Figure~\ref{fig:manual_2}, it can be inferred that approximately 50\% of the images remain aligned to the semantics of the initial sensitive prompts. The manual evaluation of the reuse attack suggests that half of the generated images retained the harmful semantics, which implies non-negligible security implication.

\begin{mdframed}[style=MyFrame,nobreak=false,align=left, userdefinedwidth=\linewidth]
        \textbf{[Key Takeaway]}: The images generated using our adversarial prompts exhibit non-negligible chances to obtain images with harmful semantic expressed in the original prompt. 
\end{mdframed}





\subsection{Eval@Cost effectiveness of Attack}
\label{sec-eval-cost}
Our proposed attack leverages LLM as the backbone to generate adversarial prompts, thus incurring relevant token costs for executing the attack. 

In the one-time attack scenario, the input token cost is divided into two categories: fixed cost and elastic cost. The fixed cost stems from helper prompts, primarily \textsc{Divide Prompts}. The elastic cost, on the other hand, mainly arises from the intermediate outputs that need to be fed into subsequent prompts. 
For the re-use attack, the input token cost is approximately equivalent to the output token cost from the previously successful one-time attacks.
% The size and complexity of helper Prompts is different.
Various commercial LLMs have distinct API pricing schemes based on token usage. We have documented the API pricing schemes of the LLMs used in our evaluation in Table~\ref{tab:llm_pricing}, where the `Words/Tokens' column represents the conversion ratio between tokens and words.

Figure~\ref{fig:cost_token}, \ref{fig:cost_money} details the token usage and associated costs (unit: U.S. dollar) for executing our attack using six different LLMs.
In accordance with the measurement standard outlined in \cite{qianwen_14_pricing}, we consider three characters as equivalent to one word. We then use various word-to-token conversion ratios shown in Table~\ref{tab:llm_pricing} to calculate the token usage for different backbone LLMs. From this, we then calculate the corresponding costs. 

Figure~\ref{fig:cost_money} shows that GPT-4 incurs a low cost of only \$0.009 in terms of fixed cost, and \$0.035 per attack. This means that with less than one dollar, it's possible to support approximately 28 attacks using GPT-4 as the backbone LLM, potentially yielding stable adversarial prompts suitable for subsequent reuse attacks (\ie, targeting web interface, not including the cost of the \dalle~3 API for image generation).
With the ongoing evolution of LLMs, the cost of API calls is becoming increasingly affordable. This trend highlights the potential security implications of using LLM-generated adversarial prompts, particularly in terms of their accessibility and cost-effectiveness for widespread use.

\begin{mdframed}[style=MyFrame,nobreak=false,align=left, userdefinedwidth=\linewidth]
        \textbf{[Key Takeaway]}: Our attack is highly cost-effective in generating adversarial prompts. With just 1 dollar, it's possible to enable 28 attack attempts using GPT-4 as the LLM backbone, and a remarkable 1000 attack attempts when employing cheaper and smaller LLM model, Qwen-14B as the backbone.
\end{mdframed}
